Numerical Stability on Local Integral Methods using RBF-QR

Many local integral methods are based on an integral formulation over small and heavilly overlapping stencils with local RBF interpolations. These functions have become an extremely effective tool for interpolation on scattered node sets, however the ill-conditioning of the interpolation matrix -- when the RBF shape parameter tends to zero corresponding to best accuracy -- is a serious task. Several stabilizing methods have been developed to deal with this near flat RBFs. The inclusion of the RBF-QR technique in the process of approximating in local integral methods makes possible to avoid this problem and stabilize the numerical error. In this paper we combine this technique in a local integral method and present accuracy results for Poisson, convection-difussion and thermal boundary layer PDEs.

==> PCP-article-references.tex <==
@BOOK{milne_thomson_68,
    Address        = {New York},
    Author         = {L.M. Milne-Thomson},
    Publisher      = {The Macmillan Company},
    Title          = {Theoretical Hydrodynamics},
    Year           = {1968}
}
@BOOK{brebbia_etall_84,
    Address        = {Berlin and New York},
    Author         = {C. A. Brebbia and J. C. F. Telles and L. C. Wrobel},
    Publisher      = {Springer-Verlag},
    Title          = {Boundary Element Techniques},
    Pages          = {11--13},
    Year           = {1984}
}
@BOOK{part_brebbia_92,
    Address        = {Southamton},
    Author         = {P. W. Partridge and C. A. Brebbia},
    Publisher      = {Elsevier Applied Science},
    Title          = {The dual reciprocity boundary element method},
    Year           = {1992}
}
@ARTICLE{kansa_carlson_95,
    Author         = {E. J. Kansa, and R. E. Carlson},
    Journal        = {Computational Fluid Dynamics},
    Pages          = {479--496},
    Title          = {Radial basis functions: a class of grid-free, scattered data approximations},
    Volume         = {3/4},
    Year           = {1995}
}
@ARTICLE{kansa_carlson_92,
    Author         = {E. J. Kansa, and R. E. Carlson},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {99--120},
    Title          = {Improved accuracy of multiquadric interpolation using variable shape parameters},
    Volume         = {24(12)},
    Year           = {1992}
}
@ARTICLE{wertz_kansa_06,
    Author         = {J. Wertz, and E. J. Kansa},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {1335--1348},
    Title          = {The role of the multiquadric shape parameters in solving partial differential equations},
    Volume         = {51(8)},
    Year           = {2006}
}
@ARTICLE{fornberg_zuev_07,
    Author         = {B. Fornberg, and J. Zuev},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {379--398},
    Title          = {The {R}unge phenomenon and spatially variable shape parameters in rbf interpolation},
    Volume         = {54(3)},
    Year           = {2007}
}
@ARTICLE{taigbenu_95,
    Author         = {A. E. Taigbenu},
    Journal        = {International Journal for Numerical Methods in Engineering},
    Pages          = {2241--2263},
    Title          = {The green element method},
    Volume         = {38(13)},
    Year           = {1995}
}
@ARTICLE{popov_power_96,
    Author         = {V. Popov and H. Power},
    Journal        = {Boundary Element Communications},
    Pages          = {1--5},
    Title          = {A domain decomposition in the dual reciprocity approach},
    Volume         = {7/1},
    Year           = {1996}
}
@ARTICLE{popov_power_99_IJNME,
    Author         = {V. Popov and H. Power},
    Journal        = {International Jounal for Numerical Methods in Engineering},
    Title          = {The {DRM-MD} integral equation method: an efficent approach for the numerical solution of domain dominant problems},
    Pages          = {327--353},
    Volume         = {44(3)},
    Year           = {1999},
}
@ARTICLE{popov_power_99_EABE,
    Author         = {V. Popov and H. Power},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {175--188},
    Title          = {The {DRM-MD} approach for the numerial solution of gas flow in porous media with application to landfill},
    Volume         = {23},
    Year           = {1999},
}
@ARTICLE{portapila_power_07,
    Author         = {M. Portapila and H. Power},
    Journal        = {International Journal for Numerical Methods in Engineering},
    Pages          = {47-65},
    Title          = {A convergence analysis of the performance of the {DRM-MD} boundary integral approach},
    Volume         = {71},
    Year           = {2007}
}
@ARTICLE{portapila_power_08,
    Author         = {M. Portapila and H. Power},
    Journal        = {Numerical Methods for Partial Differential Equations},
    Pages          = {1430-1459},
    Title          = {Iterative solution schemes for quadratic {DRM-MD}},
    Volume         = {24(6)},
    Year           = {2008}
}
@ARTICLE{orsini_power_morvan_08,
    Author         = {P. Orsini and H. Power and H. Morvan},
    Journal        = {Computer Modeling in Engineering adn Sciences},
    Pages          = {187-207},
    Title          = {Improving Volume Element Methods By Meshless Radial Basis Function Techniques},
    Volume         = {23(3)},
    Year           = {2008}
}
@ARTICLE{florez_power_chejne_00,
    Author         = {W. Florez and H. Power and F. Chejne},
    Journal        = {Communications in Numerical Methods in Engineering},
    Title          = {Multi-domain dual reciprocity BEM approach for the Navier-Stokes system of equations},
    Pages          = {671-681},
    Volume         = {16},
    Year           = {2000}
}
@ARTICLE{florez_power_02,
    Author         = {W. Florez and H. Power},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {457-472},
    Title          = {DRM multi-domain mass conservative interpolation approach for the BEM solution of the two-dimensional Navier-Stokes equations},
    Volume         = {43},
    Year           = {2002}
}
@ARTICLE{popov_bui_10,
    Author         = {V. Popov and T. T. Bui},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {680-689},
    Title          = {A meshless solution to two-dimensional convection-diffusion problems},
    Volume         = {34},
    Year           = {2010}
}
@ARTICLE{bui_popov_09,
    Author         = {T. T. Bui and V. Popov},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {456-466},
    Title          = {Domain decomposition boundary element method with overlapping sub-domains},
    Volume         = {33},
    Year           = {2009}
}
@ARTICLE{dogan_popov_ooi_12,
    Author         = {H. Dogan and V. Popov and E. H. Ooi},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {934-943},
    Title          = {The radial basis integral equation method for solving the Helmholtz equation},
    Volume         = {36},
    Year           = {2012}
}
@ARTICLE{ooi_popov_12,
    Author         = {E. H. Ooi and V. Popov},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {716-726},
    Title          = {An efficent implementation of the radial basis integral equation method},
    Volume         = {36},
    Year           = {2012}
}
@ARTICLE{ooi_popov_dogan_12,
    Author         = {E. H. Ooi and V. Popov and H. Dogan},
    Journal        = {Applied Mathematics and Computation},
    Pages          = {9470–9488},
    Title          = {Three-dimensional solution for acoustic and transport problems using the radial basis integral equation method},
    Volume         = {218(18)},
    Year           = {2012}
}
@ARTICLE{ooi_popov_12_ComMech,
    Author         = {E. H. Ooi and V. Popov},
    Journal        = {Computational Mechanics},
    Pages          = {717-729},
    Title          = {A simplified approach for imposing the boundary conditions in the local boundary integral equation method},
    Volume         = {51(5)},
    Year           = {2013}
}
@ARTICLE{ooi_popov_dogan_12,
    Author         = {E. H. Ooi, V. Popov and H. Dogan},
    Journal        = {Applied Mathematics and Computation},
    Title          = {Three-dimensional solution for acoustic and transport problems using the radial basis integral equation method},
    Year           = {2012}
}
@ARTICLE{hardy_90,
    Author         = {R. L. Hardy},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {163--208},
    Volume         = {19},    
    Title          = {Theory and applications of the multiquadrics––biharmonic method (20 years of discovery 1968–1988)},
    Year           = {1990}
}

@ARTICLE{madych_nelson_92,
    Author         = {W. R. Madych, and S. A. Nelson},
    Journal        = {Journal of Approximation Theory},
    Pages          = {94--114},
    Volume         = {70},    
    Title          = {Bounds on Multivariate Polynomials and Exponential Error Estimates for Multiquadric Interpolation},
    Year           = {1992}
}
@ARTICLE{madych_92,
    Author         = {W. R. Madych},
    Journal        = {Computer and Mathematics with Applications},
    Pages          = {121-138},
    Volume         = {24(12)},    
    Title          = {Miscellaneous Error Bounds for Multiquadric and Related Interpolators},
    Year           = {1992}
}
@ARTICLE{wu_92,
    Author         = {Z. Wu },
    Journal        = {Approximation Theory and Applications},
    Pages          = {1-11},
    Volume         = {8(2)},    
    Title          = {Hermite-Birkhoff interpoation of scattered data by radial basis function },
    Year           = {1992}
}
@ARTICLE{sun_94,
    Author         = {X. Sun},
    Journal        = {Linear Algebra Applications},
    Pages          = {135-146},
    Volume         = {207},    
    Title          = {Scattered Hermite interpolation using radial basis functions},
    Year           = {1994}
}
@ARTICLE{schaback_95,
    Author         = {R. Schaback},
    Journal        = {Advances in Computational Mathematics},
    Pages          = {251--264},
    Volume         = {3},    
    Title          = {Error estimates and condition numbers for Radial Basis Function interpolatns},
    Year           = {1995}
}
@ARTICLE{schaback_95_II,
    Author         = {R. Schaback},
    Journal        = {Approximation Theory VIII},
    Pages          = {491--514},
    Title          = {Multivariate interpolation and approximation by translates of a basis function},
    Volume         = {1},
    Year           = {1995}
}
@ARTICLE{fornberg_wright_06,
    Author         = {B. Fornberg and G. Wright},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {853-867},
    Title          = {Stable computation of multiquadric interpoations for all values of the shape parameter},
    Volume         = {48},
    Year           = {2004}
}
@ARTICLE{wright_fornberg_06,
    Author         = {G. B. Wright and B. Fornberg},
    Journal        = {Journal of Computational Physics},
    Pages          = {99-123},
    Volume         = {212},    
    Title          = {Scattered node compact finite difference-type formulas generated from radial basis functions},
    Year           = {2006}
}
@ARTICLE{golberg_etall_98,
    Author         = {M. A. Golberg, C. S. Chen,H. Bowman and H. Power},
    Journal        = {Computational Mechanics},
    Pages          = {141-148},
    Volume         = {21},    
    Title          = {Some comments on the use of radial basis functions in the dual reciprocity method},
    Year           = {1998}
}
@INCOLLECTION{nardini_brebbia_85,
    Address        = {Berlin and New York},
    Author         = {D. Nardini  and C. A. Brebbia},
    Booktitle      = {Topics in Boundary Elements Research},
    Editor         = {C. A. Brebbia},
    Pages          = {191--207},
    Publisher      = {Springer-Verlag},
    Title          = {Boundary element integral formulation of mass matrices for dynamic analysis ({C}hapter 7)},
    Year           = {1985}
}
@BOOK{brebbia_aliabadi_93,
    Address        = {Southampton and Boston},
    Editor         = {C. A. Brebbia and M. H. Aliabadi},
    Publisher      = {Computational Mechanics Publications},
    Title          = {Industrial Applications of the Boundary Element Method},
    Year           = {1993}
}
@INPROCEEDINGS{funke_84,
    Address        = {Amsterdam},
    Author         = {E. R. Funke},
    Booktitle      = {Proc. of the 1\textsuperscript{st} Int. Conf. On Hydraulic Engineering Software},
    Editor         = {C. A. Brebbia and C. Maksimovic and M. Radojkowic},
    Pages          = {1--26},
    Publisher      = {Elsevier},
    Title          = {Laboratory experimental studies controlled by mini and micro-computers},
    Year           = {1984}
}
@ARTICLE{askin_fenner_93,
    Author         = {S. Askin and R. T. Fenner},
    Journal        = {Applied Mathematical Modelling},
    Pages          = {246--245},
    Title          = {Applications  of  the  local  boundary  integral equation  technique  to  potential  problems},
    Volume         = {17 ISSN:0307-904X},
    Year           = {1993}
}
@ARTICLE{atluri_zhu_98,
    Author         = {S. N. Atluri and  T. Zhu },
    Journal        = {Computational Mechanics},
    Pages          = {117--127},
    Title          = {New Meshless Local Petrov-Galerkin {(MLPG)} approach in computational mechanics},
    Volume         = {22(2)},
    Year           = {1998}
}
@ARTICLE{zhu_zhang_atluri_98,
    Author         = {T. Zhu and J. D.  Zhang and S. N. Atluri},
    Journal        = {Computational Mechanics},
    Pages          = {223--235},
    Title          = {A local boundary integral equation {(LBIE)} method in computational mechanics, and a meshless discretization approach},
    Volume         = {21},
    Year           = {1998}
}
@ARTICLE{atluri_kim_cho_99,
    Author         = {S. N. Atluri and H. G. Kim and J. Y. Cho},
    Journal        = {Computational Mechanics },
    Pages          = {348--372},
    Title          = { A critical assessment of the truly Meshless Local Petrov-Galerkin (MLPG), and Local Boundary Integral Equation (LBIE) methods},
    Volume         = {24(5)},
    Year           = {1999}
}
@ARTICLE{sladek_sladek_atluri_00,
    Author         = { J. Sladek and V. Sladek, and S. N. Atluri},
    Journal        = {Computational Mechanics},
    Pages          = {479--496},
    Title          = {Local boundary integral equation (LBIE) method for solving problems of elasticity with nonhomogeneous material properties},
    Volume         = {24(6)},
    Year           = {2000}
}

@ARTICLE{sladek_sladek_zhang_04, 
    Author         = {J. Sladek and V. Sladek and Ch. Zhang},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {1--11},
    Title          = {A local BIEM for analysis of transient heat conduction with nonlinear source terms in FGMs},
    Volume         = {28},
    Year           = {2004}
}
@ARTICLE{guttel_pestana_14,
    Author         = {S. G\"uttel and J. Pestana},
    Issn           = {1017-1398},
    Journal        = {Numerical Algorithms},
    Title          = {Some observations on weighted GMRES},
    Pages          = {1-20},
    Year           = {2014},
    %doi           = {10.1007/s11075-013-9820-x},
    %url           = {http://dx.doi.org/10.1007/s11075-013-9820-x},
    %publisher     = {Springer US},
    %Keywords      = {Weighted GMRES; Linear systems; Krylov subspace method; Harmonic Ritz values},
    %language      = {English}
}
@ARTICLE{sellountos_polyzos_atluri_12,
    Author         = {E. J. Sellountos and D. Polyzos and S. N. Atluri},
    Journal        = {Computer Modeling in Engineering adn Sciences},
    Pages          = {513--551},
    Title          = {A New and Simple Meshless LBIE-RBF Numerical Scheme in Linear Elasticit},
    Volume         = {89(6)},
    Year           = {2012}
}
@ARTICLE{li_cheng_chen_03,
    Author         = {J. Li and A.H.-D. Cheng and C-S. Chen},
    Journal        = {Engineering Analysis with Boundary Elements},
    Pages          = {251--257},
    Title          = {On the efficiency and exponential convergence of multiquadric collocation method compared to finite element method},
    Volume         = {27(3)},
    Year           = {2003}
}
@ARTICLE{power_caruso_portapila_17,
   Author          = {H. Power and N. Caruso and M. Portapila},
   Journal         = {Engineering Analysis with Boundary Elements},
   Title           = {A note on the use of the companion solution ({D}irichlet {G}reen's function) on meshless boundary element methods},
   Pages           = {57--64},
   Volume          = {75},
   Year            = {2017},
   %doi             = {https://doi.org/10.1016/j.enganabound.2016.12.002},
   %url            = {http://www.sciencedirect.com/science/article/pii/S0955799716304970},
   %Keywords       = {DRM, Companion Solution, Green's function},
   %language       = {English}
}
@ARTICLE{caruso_portapila_power_16,
   Author          = {N. Caruso and M. Portapila and H. Power},
   Journal         = {Engineering Analysis with Boundary Elements},
   Title           = {{PDE} centres enhancement in the Localized Regular Dual Reciprocity Method},
   Pages           = {255--266},
   Volume          = {64},
   Year            = {2016},
   %issn           = {0955-7997},
   %doi            = {https://doi.org/10.1016/j.enganabound.2015.12.013},
   %url            = {http://www.sciencedirect.com/science/article/pii/S0955799715002805},
   %Keywords       = {DRM, RBF, Meshless method, Kansa interpolation},
   %language       = {English}
}
@ARTICLE{caruso_portapila_power_15,
   Author          = {N. Caruso and M. Portapila and H. Power},
   Journal         = {Computers and Mathematics with Applications},
   Title           = {An efficient and accurate implementation of the Localized Regular Dual Reciprocity Method ({LRDRM})},
   Pages           = {1342--1366},
   Volume          = {69},
   Year            = {2015},
   %doi             = {10.1016/j.camwa.2015.03.026},
   %url            = {http://dx.doi.org/10.1007/s11075-013-9820-x},
   %publisher      = {Springer US},
   %Keywords       = {Weighted GMRES; Linear systems; Krylov subspace method; Harmonic Ritz values},
   %language       = {English}
}
@ARTICLE{larsson_fornberg_03,
    Author         = {E. Larsson and B. Fornberg},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {891--902},
    Title          = {A numerical study of some radial basis function based solution methods for elliptic {PDE}s},
    Volume         = {46},
    Year           = {2003}
}
@ARTICLE{larsson_fornberg_05,
    Author         = {E. Larsson and B. Fornberg},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {103--130},
    Title          = {Theoretical and computational aspects of multivariate interpolation with increasingly flat radial basis functions},
    Volume         = {49},
    Year           = {2005}
}
@ARTICLE{fornberg_piret_07,
    Author         = {B. Fornberg and C. Piret},
    Journal        = {SIAM Journal of Scientific Computating},
    Pages          = {60--80},
    Title          = {A stable algorithm for flat radial basis functions on a sphere},
    Volume         = {30},
    Year           = {2007}
}
@ARTICLE{fornberg_zuev_07,
    Author         = {B. Fornberg and J. Zuev},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {379--398},
    Title          = {The Runge phenomenon and spatially variable shape parameters in RBF interpolation},
    Volume         = {54},
    Year           = {2007}
}
@ARTICLE{fornberg_larsson_flyer_11,
    Author         = {B. Fornberg and E. Larsson and N. Flyer},
    Journal        = {SIAM Journal of Scientific Computating},
    Pages          = {869--892},
    Title          = {Stable computation with Gaussian Radial Basis Functions},
    Volume         = {33(2)},
    Year           = {2011}
}
@ARTICLE{larsson_lehto_heryudono_fornberg_13,
    Author         = {E. Larsson and E. Lehto and A. Heryudono and B. Fornberg},
    Journal        = {SIAM Journal of Scientific Computating},
    Pages          = {A2096--A2119},
    Title          = {Stable computation of differentation matrices and scattered node stencils on Gaussian Radial Basis Functions},
    Volume         = {35(4)},
    Year           = {2013}
}
@ARTICLE{fornberg_lehto_powell_13,
    Author         = {B. Fornberg and E. Lehto and C. Powell},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {627--637},
    Title          = {Stable calculation of Gaussian-based {RBF-FD} stencils},
    Volume         = {65},
    Year           = {2013}
}
@ARTICLE{fornberg_flyer_15,
    Author         = {B. Fornberg and N. Flyer},
    Journal        = {Computers and Mathematics with Applications},
    Pages          = {531--544},
    Title          = {Fast generation of 2-{D} node distributions for mesh-free PDE discretizations},
    Volume         = {69},
    Year           = {2015}
}
@BOOK{fornber_flyer_15_book,
    Author         = {B. Fornberg and N. Flyer},
    Address        = {Philadelphia, PA, USA},
    Publisher      = {Society for Industrial and Applied Mathematics},
    Title          = {A Primer on Radial Basis Functions with Applications to the Geosciences},
    Year           = {2015}
    %Editor         = {Society for Industrial and Applied Mathematics},
}
@ARTICLE{bayona_flyer_fornberg_barnett_16,
    Author         = {V. Bayona and N. Flyer and B. Fornberg and G.A. Barnett},
    Journal        = {Journal of Computational Physics},
    Pages          = {257--273},
    Title          = {On the role of polynomials in {RBF-FD} approximations: {II}. {N}umerical solution of elliptic {PDE}s},
    Volume         = {332},
    Year           = {2017}
}
@BOOK{fasshauer_07_book,
    Author         = {G.E. Fasshauer},
    Address        = {Hackensack, NJ, USA},
    Publisher      = {World Scientific Publishing Co.},
    Title          = {Meshfree Approximation Methods with {MATLAB}},
    Year           = {2007}
    %Editor         = {World Scientific},
}
@BOOK{fasshauer_mccourt_15_book,
    Author         = {G.E. Faashauer and M. McCourt},
    Address        = {Hackensack, NJ, USA},
    Publisher      = {World Scientific Publishing Co.},
    Title          = {Kernel-based Approximation Methods using {MATLAB}},
    Year           = {2015}
    %Editor         = {World Scientific},
}
@ARTICLE{buhmann_dyn_93,
    Author         = {M. Buhmann and N. Dyn},
    Journal        = {Proceedings of the Edinburgh Mathematical Society},
    Pages          = {319--333},
    Title          = {Spectral convergence of multiquadric interpolation},
    Volume         = {36(2)},
    Year           = {1993}
}
@ARTICLE{halton_60,
    Author         = {J.H. Halton},
    Journal        = {Numerische Mathematik},
    Pages          = {84--90},
    Title          = {On the efficiency of certain quasi-random sequences of points in evaluating multi-dimensional integrals},
    Volume         = {2},
    Year           = {1960}
}
@ARTICLE{micchelli_86,
    Author         = {C.A. Michelli},
    Journal        = {Constructive Approximation},
    Pages          = {11--22},
    Title          = {Interpolation of scattered data: Distance matrices and conditionally positive definite functions},
    Volume         = {2(1)},
    Year           = {1986}
}
@ARTICLE{sandwell_87,
    Author         = {D.T. Sandwell},
    Journal        = {Geophysica Research Letters},
    Pages          = {139--142},
    Title          = {Biharmonic spline interpolation of {GEOS}-3 and {SEASAT} altimeter data},
    Volume         = {14},
    Year           = {1987}
}
@ARTICLE{deng_tang_11,
    Author         = {X. Deng and Z. Tang},
    Journal        = {Mathematical Geosciences},
    Pages          = {663--680},
    Title          = {Moving surface spline interpolation based on Green's function},
    Volume         = {43},
    Year           = {2011}
}

